Tell-XR: Conversational End-User Development of XR Automations

The availability of extended reality (XR) devices has widened their adoption, yet authoring interactive experiences remains complex for non-programmers. We introduce Tell-XR, an intelligent agent leveraging large language models (LLMs) to guide end-users in defining the interaction in XR settings using automations described as Event-Condition-Action (ECA) rules. Through a formative study, we identified the key conversation stages to define and refine automations, which informed the design of the system architecture. The evaluation study in two scenarios (a VR museum and an AR smart home) demonstrates the effectiveness of Tell-XR across different XR interaction settings.

==> bin/02-related-work.tex <==
\section{Related Work}
2 pages
\subsection{End-User Development for XR}
\ds{Preso così com'era dal deliverable. Da riassumere e inserire i riferimenti corretti}
According to Lieberman et al. [4], End-User development (EUD) includes all methods, tools, and techniques aimed at lowering the knowledge for creating or modifying software systems, enabling users without programming skills to develop new applications or adapting existing ones to their needs. Involving end-users directly in the development process can accelerate the maintenance cycle, reduce costs and accelerate the process.
Similar efforts have also been made in VR, AR, and MR, where the barrier to entry for XR development is shrinking thanks to various commercial and research authoring tools. Generally, authoring tools can be divided into two categories:
•	Desktop-based, where users create content on a standard computer screen.
•	Immersive, which allows users to develop XR experiences while they are actually inside the virtual environment.

We find different commercial/open-source desktop authoring tools for XR environments. Hubs by Mozilla [5] is a multi-user virtual platform that allows people to interact with others in VR environments and create personalized virtual rooms, by including multimedia elements or adjusting their appearance. However, the environment's behaviour remains a secondary aspect. An integrated editor 3D for Hubs, called Spoke[6], supports users in creating static representations of virtual scenes and composing 3D models. While this editor utilizes several mature techniques for end-user VR modelling in a desktop setting, it lacks robust support for defining the behaviour behind animation. Another example of a web-based application is Ottifox[7], designed to help users create VR/AR environments without writing code by using a set of rules. However, its target users are VR designers who want to create rapid prototypes, and it works only with animation. Fungus \cite{fungus} is an open-source tool for Unity, that supports novice developers to create interactive storytelling for both 2D and 3D games in Unity3D by using flowcharts. While the flowchart approach helps users to define complex behaviours, it requires a huge amount of screen, so restraining end-user developers' understanding [9] \cite{green1996usability}. 
Focusing on the customization of complex behaviours within virtual environments, different tools exist aimed at supporting end-users in customising interactions with virtual objects. Torres et al. \cite{torres2020} propose an editor where an end-user can add interactive content such as information panels, quizzes, pictures and 3D models. However, it is limited to using pre-capture 360° videos. Blecic et al. \cite{blecic2021} propose a more powerful behaviour desktop authoring tool for supporting unskilled users in creating desktop and immersive point-and-click games. It supports the user in defining the game behaviour, riddles and puzzles, by using event-condition-action (ECA) rules expressed in natural language, but also this work is limited to using pre-captured 360° photos or videos for the environment.
Generally, one limitation of desktop authoring tools, especially in VR environments, is connected to the “build-test-fix” cycle, i.e., the need to compile the entire environment to test it and verify its operation and result: this can slow down the development process, creating an additional barrier for EUDevs. The ability to manipulate the environment directly within an immersive experience makes the development more intuitive and streamlined, allowing developers to check interaction usability and user perception directly in the environment [12], [13].
The research community proposes different approaches for immersive authoring tools \cite{lee2009}, \cite{farias2022}, \cite{zhang2020flowmatic} showing the potential of this paradigm for personalising the environment and the associated interactions. However, their targets are developers. RUIS[18] is an immersive authoring toolkit that uses the metaphor of building blocks to facilitate and speed up the creation of VR experiences. While it supports a non-professional public, i.e. hobbyists and students, it requires technical knowledge to assemble the building blocks through dedicated code. VR GREP \cite{zarraonandia2016exploring} targets end-users, providing a tool where EUD can create VR environments. However, this tool does not support defining interactions or tasks, limiting it to navigation and reactions to click buttons. It is designed for novice developers, lowering the entry barrier but still requiring some technical understanding of 3D and programming concepts.

If we focus on EUD approaches exploiting Augmented Reality or Mixed Reality, one of the first contribution is Reality Editor \cite{heun2013reality}, which maps graphical elements on top of tangible interfaces associated with physical objects (e.g. push buttons or knobs). By connecting tags of different objects (by drawing a line between them), the user can create new, multi-object functionalities. However, limited attention is devoted on supporting users in flexibly specifying joint behaviour involving multiple objects. HoloFlows \cite{seiger2021} is aimed at making simpler the configuration and modelling of IoT workflows through a no-code Mixed Reality approach, by exploiting concepts from the Business Process Modelling (BPM) domain.  End users can use “virtual wires” to connect various physical IoT devices and create processes involving them.  HoloFlows requires dedicated hardware, and it is more oriented toward “wiring” objects that are physically nearby.
MagicHand [20] is an AR tool that allows end-users to control and monitor a restricted selection of IoT device behaviours using hand gestures. It first detects and localises available target devices from a depth camera mounted on the HoloLens; then, through a virtual control panel, it is able to detect and recognise hand gestures, and performs the corresponding action through a touchless interaction. 
Similar to MagicHand, HoloHome \cite{mahroo2019} targets non-developers via its AR framework for Hololens devices, in particular to support inhabitants to control real devices to carry out their activities of daily living. 
However Both MagicHand and HoloHome face similar limitations in terms of interaction complexity (i.e. they are better oriented at controlling single devices). The support provided by HoloHome to program the behaviour of various devices in a coordinated manner seems limited, as its use has been shown only in basic Ambient Assisted Living scenarios (e.g. users turning on/off a light).
Instead, Stefanidi et al. propose a collaborative platform called BricklAyeR \cite{stefanidi2019bricklayer}, an AR-based system that exploits a 3D building blocks metaphor to help non-technical users personalizing the behaviours of the mapped IoT devices. BricklAyeR allows users to define trigger-action rules through their tablets, defining how the available smart objects will respond to contextual events. Every rule is composed of triggers and actions represented as virtual blocks (i.e. 3D bricks) that can be connected like puzzle pieces: a user can direct the camera towards an object, and a ‘digital twin’ in the form of a 3D block will be created. However, it seems that this concept was not sufficiently mature to be tested with end-users, as only a cognitive walkthrough expert-based evaluation was conducted to gather feedback. The evolution of BricklAyeR has been MagiPlay \cite{stefanidi2020}, an augmented reality-based serious game for children, whose main goal is to provide young learners with an engaging way to program their surroundings. The provided user interface aims at enabling players to combine the 3D bricks as a part of the rule-based creation process. However, MagiPlay is a computational thinking learning game targeting children and mainly aiming at familiarizing them with problem-solving and computational thinking-related aspects: as such, it does not support the possibility to e.g. modify automations involving objects encountered by mobile users.
ARticulate [9] \cite{clark2022} supports a method using Snapchat-like contextual photo messages to allow users to determine available functionality and achieve their goals in one attempt with a smart space they have never seen before. However, this solution is mainly aimed at discovering functionalities, not configuring them, and it does not consider automations involving multiple connected objects. SAC \cite{ariano2023} was a first attempt to support users in controlling automations; however,it required the user to be very close to the objects to frame them and get access to the associated visualisations.  
ProInterAR \cite{ye2024} is a visual programming platform that enables novice AR creators to create immersive AR applications with a tablet and an AR-HMD, without requiring advanced programming skills. With ProInterAR users can construct interaction scenes by creating virtual content and augmenting real content from the view of an AR-HMD, and can script interactive behaviors by stacking blocks from a tablet UI; then, they can execute and control the interactions in the AR scene. While this cross-device configuration provides flexibility, potential efficiency issues could occur in this device switching.
The robot programming community explores also AR environment solutions to help end-users, for example Ikeda and Szafir propose PRogramAR[24], an AR trigger-action robot programming system designed for non-technical users.

\subsection{LLMs for automations}
The recent advances in LLMs have driven a proliferation of research works aiming at generating automations often in the form of TAP rules- using NLP-driven, conversational approaches, especially in the smart home domain [riferimenti qui].
However, the  specific challenges connected to empowering unskilled users to customise their applications in VR, AR and MR settings also exploiting LLMs  have been considered to a more limited extent.
In \cite{de2024llmr}, the authors introduce a novel framework utilizing Large Language Models (LLMs) to facilitate virtual object generation within 3D scenario development. The framework consists of five modular components with distinct functionalities: (i) Planner, which decomposes user prompts into simpler tasks; (ii) Scene Analyzer, responsible for generating a comprehensive JSON-based representation of the Unity scene the user is working on; (iii) Skill Library, tasked with retrieving pre-existing code snippets, meshes, and textural assets to solve each simpler task; (iv) Builder, designed to synthesize executable code based on Skill Library recommendations; and (v) Inspector, which performs iterative validation of generated code. The Builder and Inspector modules refine the solution in several iterative steps. Once the Inspector approves, the generated code is compiled and executed within the Unity engine, realizing the user's specified functionality.

In \cite{kurai2024}, the authors present MagicItem, a tool that integrates LLMs with scripting capabilities of the Cluster metaverse platform to enable non-programmers to define object behaviour using natural language. The tool was evaluated using online experiments with 63 users, showing that even participants with no prior programming experience could successfully create VR object behaviour, thereby showing its potential for democratizing behaviour design in VR environments. However, the system is helpful for non-programmer users performing basic behaviour, whereas limited attention has been devoted to understand to what extent the system can support unskilled users in specifying more complex behaviour, for instance dynamic behaviour of objects that should occur only when specific events and conditions happen.

AtomXR, introduced in \cite{cai2023}, is presented as a no-code immersive prototyping tool designed to address usability barriers in Extended Reality (XR) content creation. The system integrates natural language UIs powered by Large Language Models (LLMs), multimodal inputs (e.g., eye-gaze and touch interactions), and an immersive, in-headset authoring environment to enable rapid prototyping. A dedicated scripting language, AtomScript, serves as a high-level, human-readable format for developing XR applications. By allowing users to author content directly within the XR environment, AtomXR aims to eliminate the need for context switching between development and testing environments.
Empirical evaluation of the tool included two user studies, which show improvements in prototyping speed and user satisfaction compared to traditional approaches. However, the studies involved participants with varied levels of prior programming experience, thereby not specifically focusing on unskilled users; in addition, it is not clear to what extent that system is able to support complex tasks.



==> bin/cut-text.tex <==
\subsection{Walkthrough}
We describe the interaction through a compelling example in both settings



\ds{Primo esempio: Museo VR regola complessa statua Nefertiti}
%Esempio di dialogo con regola -> https://pastecode.io/s/ccm3gwms 
Following the signing of a partnership with local primary schools, the museum director asks the curator to design new interactions that mix learning and play. These interactions are meant to provide extra information about a particular artwork when a visitor places a special object into a container next to it. In this specific case, the curator is tasked with creating an interaction involving the statue of Nefertiti and a Nekhekh without clear instructions on what information to display or play.

Initially, the curator explores the environment in search of the statue. After locating it through the panel, the curator realizes that both audio speakers and a monitor are installed on the pedestal where the statue of Nefertiti stands. The curator then decides to check if any media files related to Queen Nefertiti can be used as "extra information".
The chatbot responds by listing all available media files, categorizing them as either audio or video. At this point, the curator enunciates the first part of the rule, specifying the event, placing the scepter in the container next to Nefertiti’s statue, and the resulting action, playing the file about the Egyptian queen. The chatbot confirms that it can create an automation that plays the\_egyptian\_queen.mp3 when the scepter is inside the container placed over the statue of Nefertiti, asking if the user would like to insert other conditions or events to this automation. 
The curator replies affirmatively, specifying that the visitor must also be near the statue of Queen Nefertiti. The chatbot updates the automation accordingly and summarizes the new rule. It asks if the user wants to save and export it. Upon the curator's confirmation, the chatbot generates the rule in JSON format and sends it to the Automation Engine module.

==> input/03-method.tex <==
\section{Approach}
\label{sec:method}
%Our approach leverages meta-design\cite{ardito2015,costabile2005,fischer2004} to enable user-driven customization that we demonstrate on two different points in the Mixed Reality~\cite{milgram1995} spectrum: pure VR experiences and home automation using AR to control physical devices. By structuring the system into three meta-design levels, we ensure that end-users without programming skills do not start from scratch, which would be too difficult for them~\cite{ecarules4all}, but they can easily modify and personalize their XR environments without requiring advanced technical skills.

%At the \textbf{meta-design level}, XR experts, including software developers, engineers, and designers, create the core system by providing pre-built, customizable experiences. We identify them as \textit{Element Builders}. In VR, Element Builders develop flexible immersive environments adaptable to different needs, similar to web site templates for content management systems. \textit{End User Developers} (EUDevs) personalize them including custom contents and automations defining the environment behaviour~\cite{ecarules4all}. In home automation with AR, experts handle the initial installation of the devices and provide services EUDevs can use to define automations for smart devices. The default configuration of these devices and services ensures a functional and structured starting point.

%At the \textbf{design level}, \textit{EUDevs} take advantage of expert-provided tools to modify and tailor the system to their needs. In VR, they configure template-based experiences, adjusting layouts, interactions, and content to match their specific goals. In the home automation setting, they create and refine automation rules, adapting smart home behaviours to fit their personal routines and preferences.

%Finally, at the \textbf{use level}, \textit{XR Consumers} interact with the customized system seamlessly. Whether engaging with a personalized VR experience or living in an AR-enhanced smart home, they enjoy the benefits of both expert-built and EUDev-customized content without distinguishing between the two. 

%short version
Our approach enables user-driven customization across the Mixed Reality~\cite{milgram1995} spectrum, from VR experiences to AR-based home automation. By structuring the system into three levels, we ensure non-programmers can personalize their XR environments without starting from scratch~\cite{ecarules4all}. XR experts (\textit{Element Builders}) create flexible, customizable experiences. In VR, they develop adaptable environments, while in AR home automation, they set up devices and services. \textit{End User Developers} (EUDevs) modify these systems—adjusting VR templates or defining smart home automation rules, while \textit{XR Consumers} seamlessly interact with the customized experience.

The wide range of input modalities in XR, combined with the natural language processing capabilities of LLMs, presents an opportunity to simplify automation for EUDevs. By lowering both the \textit{threshold} (knowledge needed) and \textit{ceiling} (expressiveness of automation)~\cite{myers2000}, we aim to assist EUDevs in translating their intentions into clear automation descriptions. Instead of generating code in a programming language, we represent automations as Event-Condition-Action (ECA) rules, enabling EUDevs to easily understand and modify the output to match their intentions.

ECA rules are a variant of the Trigger-Action-Programming (TAP) paradigm  “IF <a trigger occurs>, THEN <an action is executed>”. Thus, the trigger represents the \textit{event} that fires the rule, thus it involves a change of context within the environment; the \textit{action} describes the operation to execute. Additionally, a \textit{condition} could appear: in this case, when an event occurs, the system checks the condition, to evaluate whether the action should be executed or not. 

